Measurement of CP-Violating Asymmetries in B0-->(rhopi)0 Using a Time-Dependent Dalitz Plot Analysis

We report a measurement of CP-violating asymmetries in B0-->(rhopi)0-->pi+pi-pi0 decays using a time-dependent Dalitz plot analysis. The results are obtained from a data sample of 375 million Y(4S) --> BBbar decays, collected by the BaBar detector at the PEP-II asymmetric-energy B Factory at SLAC. We measure 26 coefficients of the bilinear form-factor terms occurring in the time-dependent decay rate of the B0 meson. We derive the physically relevant quantities from these coefficients. In particular, we measure a constraint on the angle alpha of the Unitarity Triangle.

==> FitResults_corrmat.tex <==
\setlength{\tabcolsep}{0.0pc}
{\small
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrrrrrrrrrrrr}
\hline
&&\\[-0.3cm]
             \rule[-6pt]{0pt}{18pt}          &     $\IM$   &     $\IP$   &    $\Uzp$   &    $\UMm$   &    $\UMp$   &    $\UPm$   & $\UPMmIm$   & $\UPMmRe$  &   $\UPMpIm$   & $\UPMpRe$   &  $\IPMIm$   &  $\IPMRe$   & $\UPzpIm$   & $\UPzpRe$   & $\UMzpIm$   \\[0.15cm]
\hline                                                                                                 &&\\[-0.3cm]
 $\IM      $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $\\
 $\IP      $&$ 0.00 $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $\\
 $\Uzp     $&$ 0.16 $&$ 0.21 $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $\\
 $\UMm     $&$ 0.03 $&$ 0.01 $&$ 0.01 $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $\\
 $\UMp     $&$ 0.01 $&$ 0.01 $&$-0.05 $&$ 0.00 $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $\\
 $\UPm     $&$-0.06 $&$-0.03 $&$ 0.01 $&$-0.03 $&$-0.06 $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $\\
 $\UPMmIm  $&$ 0.07 $&$-0.04 $&$ 0.07 $&$-0.10 $&$-0.05 $&$-0.04 $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $&$ $&$ $&$ $\\
 $\UPMmRe  $&$-0.02 $&$-0.01 $&$-0.04 $&$ 0.02 $&$ 0.01 $&$ 0.01 $&$-0.05 $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $&$ $&$ $\\
 $\UPMpIm  $&$-0.10 $&$-0.01 $&$-0.09 $&$ 0.05 $&$ 0.13 $&$ 0.13 $&$-0.05 $&$ 0.15 $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $&$ $\\
 $\UPMpRe  $&$-0.03 $&$ 0.02 $&$-0.02 $&$ 0.02 $&$-0.08 $&$ 0.07 $&$-0.01 $&$-0.01 $&$-0.03 $&$ 1.00 $&$ $&$ $&$ $&$ $&$ $\\
 $\IPMIm   $&$ 0.09 $&$-0.05 $&$ 0.06 $&$-0.10 $&$ 0.04 $&$-0.00 $&$ 0.27 $&$-0.04 $&$-0.14 $&$-0.10 $&$ 1.00 $&$ $&$ $&$ $&$ $\\
 $\IPMRe   $&$-0.02 $&$ 0.00 $&$ 0.01 $&$ 0.06 $&$ 0.03 $&$-0.02 $&$-0.02 $&$-0.04 $&$ 0.05 $&$-0.03 $&$-0.01 $&$ 1.00 $&$ $&$ $&$ $\\
 $\UPzpIm  $&$-0.07 $&$-0.00 $&$-0.18 $&$ 0.03 $&$ 0.03 $&$-0.01 $&$-0.11 $&$ 0.08 $&$ 0.06 $&$ 0.02 $&$-0.10 $&$ 0.12 $&$ 1.00 $&$ $&$ $\\
 $\UPzpRe  $&$-0.00 $&$-0.01 $&$ 0.04 $&$-0.19 $&$ 0.01 $&$ 0.00 $&$ 0.13 $&$-0.00 $&$-0.06 $&$-0.04 $&$ 0.13 $&$ 0.01 $&$-0.16 $&$ 1.00 $&$ $\\
 $\UMzpIm  $&$ 0.02 $&$-0.01 $&$ 0.13 $&$ 0.01 $&$-0.05 $&$ 0.01 $&$ 0.03 $&$-0.01 $&$-0.04 $&$ 0.04 $&$ 0.00 $&$-0.15 $&$-0.19 $&$-0.00 $&$ 1.00 $\\
 $\UMzpRe  $&$-0.05 $&$-0.05 $&$-0.05 $&$ 0.01 $&$ 0.01 $&$ 0.04 $&$-0.06 $&$ 0.03 $&$ 0.13 $&$ 0.01 $&$-0.07 $&$ 0.12 $&$ 0.14 $&$-0.05 $&$-0.01 $
\\[0.15cm]\hline			      
\end{tabular*} 
}



==> babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{{\rm \,\mum}}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees


%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
% added by GHM on March 25, 2003
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}



\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}






% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ A\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ B\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ C\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ D\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ E\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\bf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\bf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\bf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}


==> corrTableStat1.tex <==
\setlength{\tabcolsep}{0.0pc}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccccccccccccc}
\hline
 && \\[-0.3cm]
\rule[-6pt]{0pt}{18pt}  & $\sigPiNb$  &      $\Iz$  &      $\IM$  &   $\IMzIm$  &   $\IMzRe$  &      $\IP$  &   $\IPzIm$  &   $\IPzRe$  &   $\IPMIm$  &   $\IPMRe$  &     $\Uzm$  &     $\Uzp$  &  $\UMzmIm$ \\[0.15cm]
\hline
 &&\\[-0.3cm] $\sigPiNb$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  &  & \\
      $\Iz$  &  $\phantom{-}0.02$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  & \\
      $\IM$  &  $\phantom{-}0.04$  &  $-0.07$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  & \\
   $\IMzIm$  &  $\phantom{-}0.00$  &  $-0.06$  &  $\phantom{-}0.20$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  & \\
   $\IMzRe$  &  $-0.06$  &  $\phantom{-}0.16$  &  $-0.17$  &  $-0.12$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  & \\
      $\IP$  &  $-0.02$  &  $-0.01$  &  $-0.08$  &  $-0.13$  &  $\phantom{-}0.12$  &  $\phantom{-}1.00$  &  &  &  &  &  &  & \\
   $\IPzIm$  &  $\phantom{-}0.01$  &  $\phantom{-}0.03$  &  $-0.03$  &  $-0.05$  &  $\phantom{-}0.02$  &  $\phantom{-}0.27$  &  $\phantom{-}1.00$  &  &  &  &  &  & \\
   $\IPzRe$  &  $-0.01$  &  $\phantom{-}0.08$  &  $\phantom{-}0.03$  &  $\phantom{-}0.11$  &  $-0.04$  &  $-0.20$  &  $-0.36$  &  $\phantom{-}1.00$  &  &  &  &  & \\
   $\IPMIm$  &  $\phantom{-}0.07$  &  $\phantom{-}0.01$  &  $\phantom{-}0.10$  &  $-0.05$  &  $\phantom{-}0.01$  &  $\phantom{-}0.29$  &  $\phantom{-}0.10$  &  $-0.07$  &  $\phantom{-}1.00$  &  &  &  & \\
   $\IPMRe$  &  $\phantom{-}0.04$  &  $-0.01$  &  $\phantom{-}0.16$  &  $\phantom{-}0.28$  &  $-0.23$  &  $-0.32$  &  $-0.11$  &  $\phantom{-}0.21$  &  $-0.06$  &  $\phantom{-}1.00$  &  &  & \\
     $\Uzm$  &  $\phantom{-}0.04$  &  $\phantom{-}0.05$  &  $-0.00$  &  $-0.12$  &  $-0.25$  &  $-0.01$  &  $\phantom{-}0.03$  &  $-0.04$  &  $-0.00$  &  $\phantom{-}0.07$  &  $\phantom{-}1.00$  &  & \\
     $\Uzp$  &  $\phantom{-}0.17$  &  $-0.03$  &  $\phantom{-}0.09$  &  $\phantom{-}0.23$  &  $-0.09$  &  $-0.11$  &  $-0.04$  &  $\phantom{-}0.11$  &  $-0.08$  &  $\phantom{-}0.28$  &  $\phantom{-}0.04$  &  $\phantom{-}1.00$  & \\
  $\UMzmIm$  &  $-0.02$  &  $\phantom{-}0.17$  &  $-0.06$  &  $-0.01$  &  $\phantom{-}0.35$  &  $\phantom{-}0.06$  &  $\phantom{-}0.01$  &  $\phantom{-}0.00$  &  $\phantom{-}0.01$  &  $-0.11$  &  $-0.27$  &  $-0.02$  &  $\phantom{-}1.00$ \\
  $\UMzmRe$  &  $\phantom{-}0.01$  &  $-0.05$  &  $-0.05$  &  $-0.41$  &  $-0.09$  &  $\phantom{-}0.01$  &  $\phantom{-}0.01$  &  $\phantom{-}0.03$  &  $\phantom{-}0.02$  &  $\phantom{-}0.02$  &  $\phantom{-}0.11$  &  $-0.08$  &  $\phantom{-}0.02$ \\
  $\UMzpIm$  &  $-0.00$  &  $\phantom{-}0.08$  &  $-0.16$  &  $-0.37$  &  $\phantom{-}0.20$  &  $\phantom{-}0.18$  &  $\phantom{-}0.08$  &  $-0.09$  &  $\phantom{-}0.10$  &  $-0.34$  &  $\phantom{-}0.05$  &  $-0.41$  &  $\phantom{-}0.18$ \\
  $\UMzpRe$  &  $\phantom{-}0.01$  &  $\phantom{-}0.05$  &  $\phantom{-}0.01$  &  $-0.07$  &  $\phantom{-}0.05$  &  $-0.00$  &  $\phantom{-}0.00$  &  $\phantom{-}0.06$  &  $\phantom{-}0.03$  &  $\phantom{-}0.07$  &  $-0.00$  &  $-0.03$  &  $\phantom{-}0.15$ \\
     $\UMm$  &  $\phantom{-}0.06$  &  $\phantom{-}0.01$  &  $-0.01$  &  $-0.03$  &  $-0.02$  &  $-0.01$  &  $\phantom{-}0.01$  &  $\phantom{-}0.02$  &  $\phantom{-}0.01$  &  $\phantom{-}0.07$  &  $-0.01$  &  $-0.03$  &  $\phantom{-}0.09$ \\
     $\UMp$  &  $-0.05$  &  $-0.02$  &  $\phantom{-}0.00$  &  $\phantom{-}0.03$  &  $\phantom{-}0.07$  &  $-0.02$  &  $-0.06$  &  $\phantom{-}0.09$  &  $-0.05$  &  $\phantom{-}0.05$  &  $-0.02$  &  $\phantom{-}0.20$  &  $\phantom{-}0.05$ \\
  $\UPzmIm$  &  $\phantom{-}0.08$  &  $\phantom{-}0.12$  &  $-0.07$  &  $-0.17$  &  $\phantom{-}0.07$  &  $\phantom{-}0.10$  &  $\phantom{-}0.09$  &  $\phantom{-}0.02$  &  $\phantom{-}0.09$  &  $-0.20$  &  $\phantom{-}0.04$  &  $-0.24$  &  $\phantom{-}0.04$ \\
  $\UPzmRe$  &  $\phantom{-}0.06$  &  $\phantom{-}0.06$  &  $\phantom{-}0.03$  &  $\phantom{-}0.07$  &  $-0.13$  &  $-0.09$  &  $-0.15$  &  $\phantom{-}0.09$  &  $\phantom{-}0.00$  &  $\phantom{-}0.20$  &  $\phantom{-}0.09$  &  $\phantom{-}0.04$  &  $-0.07$ \\
  $\UPzpIm$  &  $-0.04$  &  $\phantom{-}0.05$  &  $-0.13$  &  $-0.29$  &  $\phantom{-}0.24$  &  $\phantom{-}0.26$  &  $\phantom{-}0.31$  &  $-0.32$  &  $\phantom{-}0.09$  &  $-0.44$  &  $-0.06$  &  $-0.37$  &  $\phantom{-}0.13$ \\
  $\UPzpRe$  &  $\phantom{-}0.07$  &  $\phantom{-}0.02$  &  $-0.02$  &  $-0.11$  &  $\phantom{-}0.04$  &  $\phantom{-}0.11$  &  $\phantom{-}0.23$  &  $-0.40$  &  $\phantom{-}0.10$  &  $-0.20$  &  $-0.03$  &  $-0.21$  &  $\phantom{-}0.02$ \\
  $\UPMmIm$  &  $-0.05$  &  $-0.05$  &  $-0.01$  &  $\phantom{-}0.07$  &  $-0.02$  &  $-0.07$  &  $-0.04$  &  $-0.03$  &  $-0.06$  &  $-0.09$  &  $-0.04$  &  $\phantom{-}0.03$  &  $-0.02$ \\
  $\UPMmRe$  &  $-0.06$  &  $\phantom{-}0.01$  &  $-0.01$  &  $\phantom{-}0.05$  &  $-0.03$  &  $-0.03$  &  $-0.02$  &  $\phantom{-}0.07$  &  $-0.06$  &  $\phantom{-}0.11$  &  $\phantom{-}0.02$  &  $\phantom{-}0.09$  &  $-0.00$ \\
  $\UPMpIm$  &  $-0.04$  &  $-0.04$  &  $-0.01$  &  $\phantom{-}0.06$  &  $-0.07$  &  $\phantom{-}0.00$  &  $\phantom{-}0.01$  &  $-0.06$  &  $\phantom{-}0.06$  &  $-0.16$  &  $-0.04$  &  $-0.02$  &  $-0.05$ \\
  $\UPMpRe$  &  $-0.10$  &  $-0.07$  &  $\phantom{-}0.03$  &  $\phantom{-}0.06$  &  $\phantom{-}0.01$  &  $-0.04$  &  $-0.02$  &  $-0.07$  &  $\phantom{-}0.03$  &  $-0.11$  &  $-0.07$  &  $-0.00$  &  $\phantom{-}0.01$ \\
     $\UPm$  &  $-0.04$  &  $\phantom{-}0.03$  &  $\phantom{-}0.01$  &  $\phantom{-}0.04$  &  $-0.05$  &  $-0.05$  &  $-0.02$  &  $\phantom{-}0.08$  &  $\phantom{-}0.01$  &  $\phantom{-}0.17$  &  $\phantom{-}0.04$  &  $\phantom{-}0.06$  &  $-0.03$ \\
[0.15cm]\hline
\end{tabular*}


==> corrTableStat2.tex <==
\setlength{\tabcolsep}{0.0pc}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccccccccc}
\hline
 && \\[-0.3cm]
\rule[-6pt]{0pt}{18pt}  &  $\UMzmRe$  &  $\UMzpIm$  &  $\UMzpRe$  &     $\UMm$  &     $\UMp$  &  $\UPzmIm$  &  $\UPzmRe$  &  $\UPzpIm$  &  $\UPzpRe$  &  $\UPMmIm$  &  $\UPMmRe$  &  $\UPMpIm$  &  $\UPMpRe$  &     $\UPm$ \\[0.15cm]
\hline
 &&\\[-0.3cm]  $\UMzmRe$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  $\UMzpIm$  &  $\phantom{-}0.25$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  &  & \\
  $\UMzpRe$  &  $\phantom{-}0.25$  &  $\phantom{-}0.12$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  & \\
     $\UMm$  &  $\phantom{-}0.17$  &  $\phantom{-}0.04$  &  $\phantom{-}0.07$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  & \\
     $\UMp$  &  $\phantom{-}0.01$  &  $\phantom{-}0.09$  &  $\phantom{-}0.04$  &  $-0.13$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  & \\
  $\UPzmIm$  &  $\phantom{-}0.04$  &  $\phantom{-}0.24$  &  $\phantom{-}0.00$  &  $\phantom{-}0.01$  &  $-0.07$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  & \\
  $\UPzmRe$  &  $\phantom{-}0.09$  &  $-0.04$  &  $\phantom{-}0.08$  &  $\phantom{-}0.05$  &  $-0.00$  &  $\phantom{-}0.26$  &  $\phantom{-}1.00$  &  &  &  &  &  &  & \\
  $\UPzpIm$  &  $\phantom{-}0.01$  &  $\phantom{-}0.40$  &  $-0.04$  &  $-0.02$  &  $-0.08$  &  $\phantom{-}0.32$  &  $-0.14$  &  $\phantom{-}1.00$  &  &  &  &  &  & \\
  $\UPzpRe$  &  $-0.03$  &  $\phantom{-}0.09$  &  $-0.02$  &  $\phantom{-}0.02$  &  $-0.26$  &  $\phantom{-}0.17$  &  $-0.09$  &  $\phantom{-}0.35$  &  $\phantom{-}1.00$  &  &  &  &  & \\
  $\UPMmIm$  &  $-0.12$  &  $-0.19$  &  $-0.10$  &  $-0.11$  &  $-0.03$  &  $-0.05$  &  $-0.07$  &  $-0.04$  &  $\phantom{-}0.03$  &  $\phantom{-}1.00$  &  &  &  & \\
  $\UPMmRe$  &  $\phantom{-}0.04$  &  $-0.05$  &  $\phantom{-}0.03$  &  $\phantom{-}0.12$  &  $\phantom{-}0.09$  &  $-0.05$  &  $\phantom{-}0.08$  &  $-0.09$  &  $-0.12$  &  $-0.01$  &  $\phantom{-}1.00$  &  &  & \\
  $\UPMpIm$  &  $-0.09$  &  $-0.17$  &  $-0.13$  &  $-0.03$  &  $-0.10$  &  $-0.02$  &  $-0.05$  &  $-0.04$  &  $\phantom{-}0.08$  &  $\phantom{-}0.35$  &  $-0.02$  &  $\phantom{-}1.00$  &  & \\
  $\UPMpRe$  &  $-0.13$  &  $-0.19$  &  $-0.10$  &  $-0.03$  &  $-0.04$  &  $-0.07$  &  $-0.15$  &  $\phantom{-}0.01$  &  $\phantom{-}0.07$  &  $\phantom{-}0.25$  &  $-0.01$  &  $\phantom{-}0.18$  &  $\phantom{-}1.00$  & \\
     $\UPm$  &  $\phantom{-}0.06$  &  $\phantom{-}0.02$  &  $\phantom{-}0.05$  &  $-0.03$  &  $\phantom{-}0.14$  &  $\phantom{-}0.11$  &  $\phantom{-}0.30$  &  $-0.09$  &  $-0.13$  &  $-0.03$  &  $\phantom{-}0.16$  &  $-0.10$  &  $-0.11$  &  $\phantom{-}1.00$ \\
[0.15cm]\hline
\end{tabular*}


==> corrTableSyst1.tex <==
\setlength{\tabcolsep}{0.0pc}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccccccccccccc}
\hline
 && \\[-0.3cm]
\rule[-6pt]{0pt}{18pt}  & $\sigPiNb$  &      $\Iz$  &      $\IM$  &   $\IMzIm$  &   $\IMzRe$  &      $\IP$  &   $\IPzIm$  &   $\IPzRe$  &   $\IPMIm$  &   $\IPMRe$  &     $\Uzm$  &     $\Uzp$  &  $\UMzmIm$ \\[0.15cm]
\hline
 &&\\[-0.3cm] $\sigPiNb$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  &  & \\
      $\Iz$  &  $\phantom{-}0.29$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  & \\
      $\IM$  &  $\phantom{-}0.12$  &  $-0.68$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  & \\
   $\IMzIm$  &  $-0.18$  &  $-0.61$  &  $\phantom{-}0.73$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  & \\
   $\IMzRe$  &  $-0.07$  &  $\phantom{-}0.84$  &  $-0.82$  &  $-0.60$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  & \\
      $\IP$  &  $\phantom{-}0.72$  &  $\phantom{-}0.18$  &  $\phantom{-}0.24$  &  $-0.03$  &  $-0.05$  &  $\phantom{-}1.00$  &  &  &  &  &  &  & \\
   $\IPzIm$  &  $\phantom{-}0.10$  &  $-0.57$  &  $\phantom{-}0.73$  &  $\phantom{-}0.75$  &  $-0.61$  &  $\phantom{-}0.40$  &  $\phantom{-}1.00$  &  &  &  &  &  & \\
   $\IPzRe$  &  $-0.28$  &  $\phantom{-}0.59$  &  $-0.66$  &  $-0.43$  &  $\phantom{-}0.62$  &  $-0.48$  &  $-0.79$  &  $\phantom{-}1.00$  &  &  &  &  & \\
   $\IPMIm$  &  $\phantom{-}0.18$  &  $\phantom{-}0.13$  &  $\phantom{-}0.14$  &  $\phantom{-}0.01$  &  $-0.08$  &  $\phantom{-}0.03$  &  $\phantom{-}0.23$  &  $-0.21$  &  $\phantom{-}1.00$  &  &  &  & \\
   $\IPMRe$  &  $\phantom{-}0.35$  &  $\phantom{-}0.12$  &  $\phantom{-}0.08$  &  $\phantom{-}0.13$  &  $-0.17$  &  $-0.09$  &  $-0.14$  &  $\phantom{-}0.38$  &  $-0.01$  &  $\phantom{-}1.00$  &  &  & \\
     $\Uzm$  &  $\phantom{-}0.79$  &  $-0.15$  &  $\phantom{-}0.41$  &  $\phantom{-}0.13$  &  $-0.49$  &  $\phantom{-}0.70$  &  $\phantom{-}0.38$  &  $-0.46$  &  $-0.10$  &  $\phantom{-}0.36$  &  $\phantom{-}1.00$  &  & \\
     $\Uzp$  &  $-0.83$  &  $-0.53$  &  $\phantom{-}0.27$  &  $\phantom{-}0.46$  &  $-0.22$  &  $-0.69$  &  $\phantom{-}0.16$  &  $\phantom{-}0.01$  &  $-0.00$  &  $-0.22$  &  $-0.66$  &  $\phantom{-}1.00$  & \\
  $\UMzmIm$  &  $-0.83$  &  $-0.28$  &  $\phantom{-}0.01$  &  $\phantom{-}0.26$  &  $\phantom{-}0.07$  &  $-0.47$  &  $\phantom{-}0.17$  &  $-0.08$  &  $\phantom{-}0.13$  &  $-0.65$  &  $-0.77$  &  $\phantom{-}0.79$  &  $\phantom{-}1.00$ \\
  $\UMzmRe$  &  $\phantom{-}0.70$  &  $\phantom{-}0.23$  &  $-0.05$  &  $-0.33$  &  $-0.13$  &  $\phantom{-}0.51$  &  $-0.07$  &  $\phantom{-}0.05$  &  $\phantom{-}0.01$  &  $\phantom{-}0.51$  &  $\phantom{-}0.72$  &  $-0.76$  &  $-0.83$ \\
  $\UMzpIm$  &  $-0.22$  &  $\phantom{-}0.21$  &  $-0.41$  &  $-0.57$  &  $\phantom{-}0.10$  &  $-0.29$  &  $-0.52$  &  $\phantom{-}0.47$  &  $-0.00$  &  $\phantom{-}0.03$  &  $-0.12$  &  $-0.09$  &  $-0.05$ \\
  $\UMzpRe$  &  $-0.39$  &  $\phantom{-}0.32$  &  $-0.43$  &  $-0.27$  &  $\phantom{-}0.55$  &  $-0.31$  &  $-0.24$  &  $\phantom{-}0.14$  &  $\phantom{-}0.31$  &  $-0.51$  &  $-0.76$  &  $\phantom{-}0.27$  &  $\phantom{-}0.60$ \\
     $\UMm$  &  $-0.36$  &  $-0.25$  &  $\phantom{-}0.12$  &  $\phantom{-}0.05$  &  $-0.22$  &  $-0.39$  &  $-0.06$  &  $\phantom{-}0.04$  &  $\phantom{-}0.05$  &  $-0.08$  &  $-0.22$  &  $\phantom{-}0.40$  &  $\phantom{-}0.30$ \\
     $\UMp$  &  $\phantom{-}0.48$  &  $\phantom{-}0.57$  &  $-0.40$  &  $-0.45$  &  $\phantom{-}0.24$  &  $\phantom{-}0.36$  &  $-0.32$  &  $\phantom{-}0.42$  &  $-0.05$  &  $\phantom{-}0.47$  &  $\phantom{-}0.44$  &  $-0.73$  &  $-0.68$ \\
  $\UPzmIm$  &  $\phantom{-}0.30$  &  $\phantom{-}0.42$  &  $-0.24$  &  $-0.51$  &  $\phantom{-}0.28$  &  $\phantom{-}0.04$  &  $-0.25$  &  $\phantom{-}0.11$  &  $\phantom{-}0.55$  &  $-0.03$  &  $-0.09$  &  $-0.27$  &  $-0.15$ \\
  $\UPzmRe$  &  $-0.61$  &  $-0.29$  &  $-0.01$  &  $-0.08$  &  $-0.24$  &  $-0.76$  &  $-0.34$  &  $\phantom{-}0.38$  &  $\phantom{-}0.03$  &  $\phantom{-}0.12$  &  $-0.45$  &  $\phantom{-}0.57$  &  $\phantom{-}0.31$ \\
  $\UPzpIm$  &  $-0.57$  &  $-0.37$  &  $\phantom{-}0.04$  &  $\phantom{-}0.01$  &  $-0.06$  &  $-0.18$  &  $\phantom{-}0.22$  &  $-0.37$  &  $\phantom{-}0.01$  &  $-0.84$  &  $-0.40$  &  $\phantom{-}0.47$  &  $\phantom{-}0.77$ \\
  $\UPzpRe$  &  $\phantom{-}0.40$  &  $\phantom{-}0.15$  &  $\phantom{-}0.10$  &  $-0.02$  &  $\phantom{-}0.15$  &  $\phantom{-}0.34$  &  $\phantom{-}0.25$  &  $-0.50$  &  $\phantom{-}0.45$  &  $-0.35$  &  $\phantom{-}0.02$  &  $-0.18$  &  $\phantom{-}0.04$ \\
  $\UPMmIm$  &  $-0.17$  &  $-0.20$  &  $\phantom{-}0.22$  &  $\phantom{-}0.61$  &  $\phantom{-}0.02$  &  $\phantom{-}0.20$  &  $\phantom{-}0.57$  &  $-0.35$  &  $-0.15$  &  $-0.28$  &  $-0.07$  &  $\phantom{-}0.22$  &  $\phantom{-}0.40$ \\
  $\UPMmRe$  &  $\phantom{-}0.45$  &  $\phantom{-}0.53$  &  $-0.25$  &  $-0.01$  &  $\phantom{-}0.36$  &  $\phantom{-}0.45$  &  $-0.03$  &  $\phantom{-}0.33$  &  $-0.20$  &  $\phantom{-}0.48$  &  $\phantom{-}0.35$  &  $-0.56$  &  $-0.53$ \\
  $\UPMpIm$  &  $-0.89$  &  $-0.54$  &  $\phantom{-}0.19$  &  $\phantom{-}0.31$  &  $-0.28$  &  $-0.68$  &  $\phantom{-}0.12$  &  $-0.04$  &  $\phantom{-}0.06$  &  $-0.38$  &  $-0.64$  &  $\phantom{-}0.88$  &  $\phantom{-}0.84$ \\
  $\UPMpRe$  &  $\phantom{-}0.56$  &  $\phantom{-}0.20$  &  $\phantom{-}0.00$  &  $\phantom{-}0.13$  &  $\phantom{-}0.18$  &  $\phantom{-}0.70$  &  $\phantom{-}0.28$  &  $-0.30$  &  $-0.29$  &  $\phantom{-}0.00$  &  $\phantom{-}0.50$  &  $-0.55$  &  $-0.37$ \\
     $\UPm$  &  $-0.04$  &  $\phantom{-}0.56$  &  $-0.54$  &  $-0.44$  &  $\phantom{-}0.44$  &  $-0.16$  &  $-0.53$  &  $\phantom{-}0.65$  &  $-0.02$  &  $\phantom{-}0.30$  &  $-0.13$  &  $-0.23$  &  $-0.18$ \\
[0.15cm]\hline
\end{tabular*}


==> corrTableSyst2.tex <==
\setlength{\tabcolsep}{0.0pc}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccccccccc}
\hline
 && \\[-0.3cm]
\rule[-6pt]{0pt}{18pt}  &  $\UMzmRe$  &  $\UMzpIm$  &  $\UMzpRe$  &     $\UMm$  &     $\UMp$  &  $\UPzmIm$  &  $\UPzmRe$  &  $\UPzpIm$  &  $\UPzpRe$  &  $\UPMmIm$  &  $\UPMmRe$  &  $\UPMpIm$  &  $\UPMpRe$  &     $\UPm$ \\[0.15cm]
\hline
 &&\\[-0.3cm]  $\UMzmRe$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  $\UMzpIm$  &  $\phantom{-}0.33$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  &  & \\
  $\UMzpRe$  &  $-0.54$  &  $-0.07$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  &  & \\
     $\UMm$  &  $-0.34$  &  $\phantom{-}0.22$  &  $\phantom{-}0.02$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  &  & \\
     $\UMp$  &  $\phantom{-}0.80$  &  $\phantom{-}0.50$  &  $-0.41$  &  $-0.31$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  &  & \\
  $\UPzmIm$  &  $\phantom{-}0.22$  &  $\phantom{-}0.21$  &  $\phantom{-}0.32$  &  $\phantom{-}0.10$  &  $\phantom{-}0.18$  &  $\phantom{-}1.00$  &  &  &  &  &  &  &  & \\
  $\UPzmRe$  &  $-0.15$  &  $\phantom{-}0.60$  &  $\phantom{-}0.07$  &  $\phantom{-}0.49$  &  $-0.15$  &  $\phantom{-}0.11$  &  $\phantom{-}1.00$  &  &  &  &  &  &  & \\
  $\UPzpIm$  &  $-0.55$  &  $\phantom{-}0.17$  &  $\phantom{-}0.40$  &  $\phantom{-}0.27$  &  $-0.52$  &  $-0.10$  &  $\phantom{-}0.17$  &  $\phantom{-}1.00$  &  &  &  &  &  & \\
  $\UPzpRe$  &  $-0.20$  &  $-0.59$  &  $\phantom{-}0.48$  &  $-0.16$  &  $-0.37$  &  $\phantom{-}0.42$  &  $-0.54$  &  $\phantom{-}0.10$  &  $\phantom{-}1.00$  &  &  &  &  & \\
  $\UPMmIm$  &  $-0.48$  &  $-0.70$  &  $\phantom{-}0.10$  &  $-0.19$  &  $-0.39$  &  $-0.53$  &  $-0.56$  &  $\phantom{-}0.21$  &  $\phantom{-}0.23$  &  $\phantom{-}1.00$  &  &  &  & \\
  $\UPMmRe$  &  $\phantom{-}0.48$  &  $-0.20$  &  $-0.30$  &  $-0.51$  &  $\phantom{-}0.65$  &  $-0.08$  &  $-0.55$  &  $-0.69$  &  $-0.13$  &  $\phantom{-}0.21$  &  $\phantom{-}1.00$  &  &  & \\
  $\UPMpIm$  &  $-0.68$  &  $\phantom{-}0.21$  &  $\phantom{-}0.30$  &  $\phantom{-}0.48$  &  $-0.62$  &  $-0.24$  &  $\phantom{-}0.68$  &  $\phantom{-}0.68$  &  $-0.28$  &  $\phantom{-}0.09$  &  $-0.72$  &  $\phantom{-}1.00$  &  & \\
  $\UPMpRe$  &  $\phantom{-}0.20$  &  $-0.62$  &  $-0.19$  &  $-0.47$  &  $\phantom{-}0.18$  &  $-0.27$  &  $-0.91$  &  $-0.28$  &  $\phantom{-}0.35$  &  $\phantom{-}0.60$  &  $\phantom{-}0.61$  &  $-0.68$  &  $\phantom{-}1.00$  & \\
     $\UPm$  &  $\phantom{-}0.20$  &  $\phantom{-}0.48$  &  $-0.02$  &  $\phantom{-}0.34$  &  $\phantom{-}0.56$  &  $\phantom{-}0.30$  &  $\phantom{-}0.19$  &  $-0.29$  &  $-0.36$  &  $-0.33$  &  $\phantom{-}0.31$  &  $-0.17$  &  $-0.14$  &  $\phantom{-}1.00$ \\
[0.15cm]\hline
\end{tabular*}


==> covTableQ2B.tex <==
\setlength{\tabcolsep}{0.0pc}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccc}
\hline
 && \\[-0.3cm]
\rule[-6pt]{0pt}{18pt}  &     $\Acp$  &       $\C$  &      $\dC$  &       $\S$  &      $\dS$  &     $\Czz$  &     $\Szz$  &     $\fzz$ \\[0.15cm]
\hline
 &&\\[-0.3cm]     $\Acp$  &  $\phantom{-}2.57$  &  &  &  &  &  &  & \\
       $\C$  &  $-0.167$  &  $\phantom{-}9.05$  &  &  &  &  &  & \\
      $\dC$  &  $\phantom{-}0.06$  &  $\phantom{-}4.40$  &  $\phantom{-}15.55$  &  &  &  &  & \\
       $S$  &  $-0.568$  &  $-1.450$  &  $-1.961$  &  $\phantom{-}13.38$  &  &  &  & \\
      $\dS$  &  $\phantom{-}0.23$  &  $-1.389$  &  $-6.109$  &  $\phantom{-}3.97$  &  $\phantom{-}19.80$  &  &  & \\
     $\Czz$  &  $-9.758$  &  $-11.397$  &  $-10.225$  &  $\phantom{-}11.62$  &  $\phantom{-}18.32$  &  $\phantom{-}277.90$  &  & \\
     $\Szz$  &  $-0.375$  &  $\phantom{-}1.03$  &  $\phantom{-}6.73$  &  $-3.778$  &  $-3.805$  &  $\phantom{-}17.28$  &  $\phantom{-}8.77$  & \\
     $\fzz$  &  $\phantom{-}0.14$  &  $-0.086$  &  $-0.297$  &  $-0.438$  &  $-1.310$  &  $-17.007$  &  $-2.524$  &  $\phantom{-}1.49$ \\
[0.15cm]\hline
\end{tabular*}

